Run-Time Accuracy Reconfigurable Stochastic Computing for Dynamic Reliability and Power Management

In this paper, we propose a novel accuracy-reconfigurable stochastic computing (ARSC) framework for dynamic reliability and power management. Different than the existing stochastic computing works, where the accuracy versus power/energy trade-off is carried out in the design time, the new ARSC design can change accuracy or bit-width of the data in the run-time so that it can accommodate the long-term aging effects by slowing the system clock frequency at the cost of accuracy while maintaining the throughput of the computing. We validate the ARSC concept on a discrete cosine transformation (DCT) and inverse DCT designs for image compressing/decompressing applications, which are implemented on Xilinx Spartan-6 family XC6SLX45 platform. Experimental results shows that the new design can easily mitigate the long-term aging induced effects by accuracy trade-off while maintaining the throughput of the whole computing process using simple frequency scaling. We further show that one-bit precision loss for input data, which translated to 3.44dB of the accuracy loss in term of Peak Signal to Noise Ratio for images, we can sufficiently compensate the NBTI induced aging effects in 10 years while maintaining the pre-aging computing throughput of 7.19 frames per second. At the same time, we can save 74\% power consumption by 10.67dB of accuracy loss. The proposed ARSC computing framework also allows much aggressive frequency scaling, which can lead to order of magnitude power savings compared to the traditional dynamic voltage and frequency scaling (DVFS) techniques.

==> motivation.tex <==
\section{Motivation and Background}
\label{sec:motivation}

\subsection{Conventional Stochastic Multiplication}
\label{sec:Conv SC Mul}



\begin{figure}[!htb]
\centering
\subfigure[]{
\label{fig:subfig:a}
\includegraphics[width=0.85\columnwidth]{figs/conv_rng.eps}}
\subfigure[]{
\label{fig:subfig:b}
\includegraphics[width=0.85\columnwidth]{figs/conv_sc_mul.eps}}
\caption{(a) Conventional SNG. (b) Conventional Stochastic Multiplication.}
\label{fig:Conv SC and SNG}
\end{figure}

\subsection{State-of-The-Art Stochastic Multiplication}
\label{sec:State-of-The-Art Stochastic Multiplication}

The conventional stochastic multiplication with a very long bit-streams length, often takes
a large amount of time which is proportional to the length of bit-streams to complete calculation. 
To improve this, authors in~\cite{Sim:DAC'18} proposed a new method called BISC-MVM, which 
significantly the process time of stochastic multiplication by using a novel SNG (Stochastic 
Number Generator). Also, different from the conventional way of generating random bit-streams, 
the BISC-MVM follows a deterministic pattern. Thus, avoids the random noise introduced by the 
random bit-streams. As illustrated in Fig.~\ref{fig:SC_mul_SNG}, the proposed SNG is composed of  
a finite state machine (FSM) and a multiplexer (MUX). The bit-stream pattern generated by the BISC-MVM 
is shown in the figure. We explain it with an example.

Suppose we have an unsigned $n$-bit binary number (BN), $x$ = $x_{n-1}$$x_{n-2}$...$x_0$, and convert it 
to a $2^n$ bits bit-stream $S$. The $x$ is multiplied by another number $w$, which is in the 
range [0,1]. To do the multiplication, first, we need to scale $w$ by a scaling factor $2^n$ to achieve 
$w_s$ = $w\cdot2^n$. Then, the $w_s$ is transformed to a bit sequence of 1's followed by 0's in the unary 
number generator (UNG), which is highlighted with green wire frame in the Fig.~\ref{fig:SC_mul_SNG}. 
The UNG is equipped with a down-counter and a comparator. 

The $(n-i)^th$ bit $x_{n-i}$ of $x$, appears firstly at $2^{i-1}$$th$ bit in $S$, then every $2^i$$th$ bit in 
$S$. When it comes to the last bit of $S$, it's always zero to make sure the value is less than one
~\cite{Sim:DAC'18}. 

\begin{figure}[!htb]
%\vspace{-0.2in}
\centering
\includegraphics[width=0.85\columnwidth]{figs/SC_mul_SNG.eps}
\caption{Stochastic multiplication module}
\label{fig:SC_mul_SNG}
%\vspace{-0.2in}
\end{figure}



==> rela_works.tex <==
\section{Related Works}
\label{sec:rela_works}


